$VH+\text{jet}$ production in hadron-hadron collisions up to order $\alpha_s^3$ in perturbative QCD

We present precise predictions for the hadronic production of an on-shell Higgs boson in association with a leptonically decaying gauge boson and a jet up to order $\alpha_s^3$. We include the complete set of NNLO QCD corrections to both charged- and neutral-current Drell-Yan type contributions, as well as the previously known leading heavy quark loop induced contributions which involve a direct Higgs-quark coupling. As an application, we study a range of differential observables in proton-proton collisions at $\sqrt{s} = 13~\text{TeV}$ for both the charged- and neutral-current production modes. For each Higgs production process, we assess the improvement in the theoretical uncertainty for both the exclusive ($n_{\text{jet}} = 1$) and inclusive ($n_{\text{jet}} \geq 1$) jet categories. We find that the inclusion of the NNLO corrections to the Drell-Yan type contributions is essential in stabilising the predictions and in reducing the theoretical uncertainty for both inclusive and exclusive jet production for all three modes. This is particularly true in the kinematical regimes associated with low to medium values of the transverse momentum of the produced vector boson and where the differential cross sections are the largest. For the neutral-current process, we find that the heavy quark loop induced contributions have their largest phenomenological impact (an increase in the size of the NNLO corrections, a distortion of the distribution shape and an enlargement of the left over remaining uncertainties) in kinematical regions associated to large values of $p_{T,Z}$ (typically above $150~\text{GeV}$) where the cross sections are smaller.

==> fig.tex <==
% Some definitions
\makeatletter

\newif\ifstartcompletesineup
\newif\ifendcompletesineup
\pgfkeys{
    /pgf/decoration/.cd,
    start up/.is if=startcompletesineup,
    start up=true,
    start up/.default=true,
    start down/.style={/pgf/decoration/start up=false},
    end up/.is if=endcompletesineup,
    end up=true,
    end up/.default=true,
    end down/.style={/pgf/decoration/end up=false}
}
\pgfdeclaredecoration{complete sines}{initial}
{
    \state{initial}[
        width=+0pt,
        next state=upsine,
        persistent precomputation={
            \ifstartcompletesineup
                \pgfkeys{/pgf/decoration automaton/next state=upsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5*\pgfdecoratedinputsegmentlength / (ceil(0.5* \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) )
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.499)
                    }
                \fi
            \else
                \pgfkeys{/pgf/decoration automaton/next state=downsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5* \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.4999)
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) )
                    }
                \fi
            \fi
            \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
        }] {}
    \state{downsine}[width=\pgfdecorationsegmentlength,next state=upsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
    }
    \state{upsine}[width=\pgfdecorationsegmentlength,next state=downsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
}
    \state{final}{}
}


\pgfdeclaredecoration{spring}{initial}
{
  \state{initial}[
    width=+0pt,
    next state=coil,
    persistent precomputation={
      \pgfmathsetmacro\matchinglength{
        (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) - \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) > 0.5
        ? (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (floor(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
        : (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
      }
      \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
    },
  ]{}
  \state{coil}[
    switch if less than=%
      0.5\pgfdecorationsegmentlength%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude to last,
    width=+\pgfdecorationsegmentlength,
  ]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{ 1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{ 2}}
    {\pgfpoint@oncoil{1    }{ 1    }{ 3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{ 4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{ 5}}
    {\pgfpoint@oncoil{2    }{ 0    }{ 6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{ 7}}
    {\pgfpoint@oncoil{1.555}{-1    }{ 8}}
    {\pgfpoint@oncoil{1    }{-1    }{ 9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}{}
}



\tikzset{
      % style to apply some styles to each segment of a path
      on each segment/.style={
        decorate,
        decoration={
          show path construction,
          moveto code={
          },
          lineto code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
          curveto code={
            \path [#1] (\tikzinputsegmentfirst)
            .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..
            (\tikzinputsegmentlast);
          },
          closepath code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
        },
      },
    % vector (old)
    vector/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start up}},
    % vector2 (old)
    vector2/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start down}},
    % gluon (old)
    gluon/.style={line join=round, line cap=round, line width=0.1+#1*0.02*\tikz@node@distance, decorate, decoration={spring, amplitude=#1*0.1*\tikz@node@distance, segment length=#1*0.18*\tikz@node@distance, aspect=#1*0.66}},
    gluon/.default=1.0,
    % Quark style: scalable arrowheads (properly centered)
    quark/.style args={#1}{
        line join=round,
        line cap=round,
        line width=0.1+0.02*\tikz@node@distance,
        postaction={
            on each segment={
                decorate,
                decoration={
                    markings,
                    % position = midpath + half of arrowhead length
                    mark=at position (0.5*\pgfdecoratedpathlength+0.08*#1*\tikz@node@distance) with
                    \arrow{Stealth[length={#1*0.16*\tikz@node@distance}, width={#1*0.14*\tikz@node@distance}]}
                }
            }
        }
    },
    quark/.default={1.0},
    % Top quark (thick quark, default arrowheads are 1.2x quark)
    tquark/.style={quark={#1}, line width=0.1+0.06*\tikz@node@distance},
    tquark/.default={1.2},
    % Quark line without arrowheads
    qline/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance},
    % Higgs line
    higgs/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, dashed}
}


\newcommand\myaction{}


% VHJ Feynman diagrams

% VHJ Born: Drell--Yan-like
\newcommand{\BornVHJ}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (tV) -- ++(-90:#2) coordinate (gt2) -- ++(-180:#2) coordinate (gt3);
        \draw [gluon] (gt2) -- ++(0:#2);
        \draw [vector] (tV) -- ++(0:0.75*#2) coordinate (VH);
        \draw [vector] (VH) -- ++(45:0.75*#2) coordinate (Vl);
        \draw [higgs] (VH) -- ++(-45:#2);
        \draw [quark] (Vl)++(75:0.75*#2) -- (Vl) -- ++(15:0.75*#2);
        \coordinate (label) at ($(tV)!0.5!(gt3)$);
    }
}

% Top loop RI VHJ (included)
\newcommand{\TopRI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (qV) -- ++(-90:1.5*#2) coordinate (qg2) -- ++(180:#2);
        \draw [vector] (qV) -- ++(0:0.85*#2) coordinate (Vl);
        \draw [gluon] (qg2) -- ++(0:0.85*#2) coordinate (g1t);
        \draw [tquark] (g1t) -- ++(30:#2) coordinate (g2t) -- ++(-90:#2) coordinate (Ht) -- (g1t);
        \draw [gluon] (g2t) -- ++(0:#2);
        \draw [higgs] (Ht) -- ++(0:#2);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (label) at ($(g1t)+({sqrt(3)/4*#2},0)$);
        \node[xshift=0.12*#2] at (label) {$\Pqt$};
    }
}


% Top loop RRI VHJ (OpenLoops has it, we cannot: corresponing VV are unknown)
\newcommand{\TopRRI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (qV) -- ++(-90:0.75*#2) coordinate (qg1) -- ++(-90:0.75*#2) coordinate (qg2) -- ++(180:#2);
        \draw [vector] (qV) -- ++(0:0.85*#2) coordinate (Vl);
        \draw [gluon] (qg2) -- ++(0:0.85*#2) coordinate (g1t);
        \draw [gluon] (qg1) -- ++(0:0.85*#2);
        \draw [tquark] (g1t) -- ++(30:#2) coordinate (g2t) -- ++(-90:#2) coordinate (Ht) -- (g1t);
        \draw [gluon] (g2t) -- ++(0:#2);
        \draw [higgs] (Ht) -- ++(0:#2);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (label) at ($(g1t)+({sqrt(3)/4*#2},0)$);
        \node[xshift=0.12*#2] at (label) {$\Pqt$};
    }
}


% Genuine (only Yukawa) two-loop correction to VHJ
\newcommand{\TopRVI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (qV) -- ++(-90:#2) coordinate (qg1) -- ++(-90:#2) coordinate (qg2) -- ++(180:#2);
        \draw [gluon] (qg1) -- ++(0:#2) coordinate (tg1);
        \draw [gluon] (qg2) -- ++(0:#2) coordinate (tg2);
        \draw [tquark] (tg2) -- (tg1) -- ++(0:#2) coordinate (tg3) -- ++(-90:#2) coordinate (tH) -- cycle;
        \draw [gluon] (tg3) -- ++(0:#2);
        \draw [higgs] (tH) -- ++(0:#2);
        \draw [vector] (qV) -- ++(0:#2) coordinate (Vl);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (label) at ($(tg1)!0.5!(tH)$);
        \node at (label) {$\Pqt$};
    }
}


% VHJ Top loop Yukawa-induced (pentagon, included)
\newcommand{\TopZHJI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [gluon] (0,0) -- ++(0:#2) coordinate (g1t);
        \draw [tquark] (g1t) -- ++(18:#2) coordinate (tV) -- ++(-54:#2) coordinate (tH) -- ++(-126:#2) coordinate (g2t) -- ++(-198:#2) coordinate (g3t) -- cycle;
        \draw [gluon] (g2t) -- ++(0:#2);
        \draw [gluon] (g3t) -- ++(0:-#2);
        \draw [vector2] (tV) -- ++(0:0.85*#2) coordinate (Vl);
        \draw [higgs] (tH) -- ++(0:#2);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (mid) at ($(g3t)!0.5!(g1t)$);
        \coordinate (label) at ($(mid)!0.5!(tH)$);
        \node [xshift=-0.05*#2] at (label) {$\Pqt$};
    }
}


% VHJ Top loop Drell--Yan-like (box, included)
\newcommand{\TopZHJII}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [gluon] (0,0) -- ++(0:#2) coordinate (gt1);
        % \draw [tquark] (gt1) -- ++(0:#2) coordinate (tV) -- ++(-90:#2) coordinate (gt2) -- ++(-180:#2) coordinate (gt3) -- cycle;
        \draw [quark] (gt1) -- ++(0:#2) coordinate (tV) -- ++(-90:#2) coordinate (gt2) -- ++(-180:#2) coordinate (gt3) -- cycle;
        \draw [gluon] (gt2) -- ++(0:#2);
        \draw [gluon] (gt3) -- ++(0:-#2);
        \draw [vector] (tV) -- ++(0:0.75*#2) coordinate (VH);
        \draw [vector] (VH) -- ++(45:0.75*#2) coordinate (Vl);
        \draw [higgs] (VH) -- ++(-45:#2);
        \draw [quark] (Vl)++(75:0.75*#2) -- (Vl) -- ++(15:0.75*#2);
        \coordinate (label) at ($(tV)!0.5!(gt3)$);
        % \node at (label) {$\Pqt/\Pqb$};
        \node at (label) {$\Pq$};
    }
}


\newcommand{\VHJrrB}[4][0]{\tikz[node distance=#4, baseline=#1]
    {
    \draw [quark] (0,0) -- ++(0:#4) coordinate (qg1) -- ++(-90:1.5*#4) coordinate (qV) -- ++(-180:#4);
    \draw [vector] (qV) -- ++(0:0.75*#4) coordinate (VH);
    \draw [vector] (VH) -- ++(30:0.85*#4) coordinate (Vl);
    \draw [higgs] (VH) -- ++(-30:{(0.85+cos(22.5)*0.75)*#4});
    \draw [quark] (Vl)++(52.5:0.75*#4) -- (Vl) -- ++(7.5:0.75*#4);
    \path (qg1)++(-90:0.5*#4) coordinate (qg2);
    \path (qg2)++(-90:0.5*#4) coordinate (qg3);

    % Draw gluon radiation if 1 < #2
    \path \pgfextra{\ifthenelse{0 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg1) -- ++(15:#4);

    % Draw second gluon radiation if 1 < #2
    \path \pgfextra{\ifthenelse{0 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg3) -- ++(15:#4);

    % Draw gluon radiation if 2 < #2
    \path \pgfextra{\ifthenelse{1 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg2) -- ++(15:#4);


    % Draw gluon loop if 0 < #3
    \path (qV)++(-180:0.7*#4) coordinate (qgl);
    \path (qg2)++(90:0.1*#4) coordinate (qgl2);
    \path \pgfextra{\ifthenelse{0 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qgl2) to [bend right=45] (qgl);

    % Draw another one if 1 < #3 (manual adjustions, duh...)
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg3)++(-90:0.16*#4) arc (-90:0:0.56*#4) coordinate (new);
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (new) arc (0:90:0.56*#4);
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (new)++(15:#4) -- ($(new)+(-10:0.03*#4)$);

    }
}

